The Bandit Whisperer: Communication Learning for Restless Bandits

Applying Reinforcement Learning (RL) to Restless Multi-Arm Bandits (RMABs) offers a promising avenue for addressing allocation problems with resource constraints and temporal dynamics. However, classic RMAB models largely overlook the challenges of (systematic) data errors - a common occurrence in real-world scenarios due to factors like varying data collection protocols and intentional noise for differential privacy. We demonstrate that conventional RL algorithms used to train RMABs can struggle to perform well in such settings. To solve this problem, we propose the first communication learning approach in RMABs, where we study which arms, when involved in communication, are most effective in mitigating the influence of such systematic data errors. In our setup, the arms receive Q-function parameters from similar arms as messages to guide behavioral policies, steering Q-function updates. We learn communication strategies by considering the joint utility of messages across all pairs of arms and using a Q-network architecture that decomposes the joint utility. Both theoretical and empirical evidence validate the effectiveness of our method in significantly improving RMAB performance across diverse problems.

==> text/1-Introduction.tex <==
\section{Introduction}

%Restless Multi-Arm Bandits (RMABs) is a multi-agent constrained resource allocation problem. This model has been successfully applied to a range of real-world problems, such as healthcare, online advertising, and anti-poaching
Restless Multi-Arm Bandits (RMABs) have been successfully applied to a range of  multi-agent constrained resource allocation problems, such as healthcare, online advertising, and anti-poaching~\cite{ruiz2020multi,lee2019optimal,hodge2015asymptotic,mate2022field,modi2019transfer,zhao2007myopic,bagheri2015restless,tripathi2019whittle}.  
In classical RMABs, there are a fixed number of arms, each may be described as an MDP
%associated with a known Markov Decision Process (MDP) 
with two actions (active and passive). At each timestep, constrained by the global budget, the RMAB strategically selects a subset of arms to play the active action with the objective of maximizing long-term accumulated rewards. 
%This selection is constrained by a global limit on the number of active actions in a timestep. 
Although finding an exact RMAB solution is PSPACE-hard~\cite{papadimitriou1994complexity}, the whittle index solution is known to be near optimal~\cite{whittle1988restless,weber1990index} in this situation. Beyond classical RMABs, important applications of RMABs involve more complex systems with multiple actions, continuous state spaces, and arms opting in and out of the system.  Recent studies have explored a variety of methods to address these challenges~\cite{hawkins2003langrangian,killian2021beyond,verloop2016asymptotically,zayas2019asymptotically,ghosh2023indexability}, with deep Reinforcement Learning (RL) emerging as a particularly effective approach, achieving state-of-the-art results across various RMAB settings ~\cite{zhao2023towards,xiong2023finite,wang2023scalable,killian2022restless}.

Unfortunately, these previous studies consider RMAB models where the reward data can be collected from every arm reliably. In real-world scenarios  modeled via RMABs, such as maternal healthcare~\cite{biswas2021learn,vermagroup, behari2024decision} and SIS epidemic model concerning COVID intervention~\cite{yaesoubi2011generalized}, each arm represents a different entity, which could be a beneficiary or a geographical region, where data collection protocols are potentially different. Different arms may be affected by noise caused by
%typically involve unreliable data sources vulnerable to 
\textbf{systematic errors} that arise due to the following practical reasons. \textbf{(1) Variability in data collection and handling protocols.}  There may be differences in data collection in different arms (entities), e.g., differences in the frequency and quality of data collected, in worker awareness or standards for data preprocessing, 
cleaning, and digitization. This variability represents sampling bias~\cite{paulus2023reinforcing} and may cause systematic errors~\cite{dubrow2022local} in some arms. For example, in maternal care, specific data collection approaches may cause systematic overestimation of expected delivery dates~\cite{fulcher2020errors}.
\textbf{(2) Data integrity and privacy.} For example, when data is gathered through surveys, topical or political bias~\cite{paulus2023reinforcing} can introduce systematic errors in some arms due to influence of authorities or impacted populations
(e.g., keeping the number of COVID cases low \cite{paulus2023reinforcing}). Additionally, driven by the principle of differential privacy, noise might be intentionally added to the data~\cite{dwork2014algorithmic}.
%\textbf{(1) Variability in data collection and handling protocols.} In some problems like 
%ARMMAN 
%maternal healthcare~\cite{biswas2021learn} and SIS epidemic model concerning COVID intervention~\cite{yaesoubi2011generalized}, each arm represents a different entity, which could be a beneficiary or a geographical region. These entities differ in the frequency and quality of data collection, merging from potentially different programs/repositories, cleaning, and digitization. This variability represents sampling bias~\cite{paulus2023reinforcing}, causes systematic errors~\cite{dubrow2022local} due to disparities in worker awareness or standards for data preprocessing, duplicate filtering, accuracy checks, etc., and results in some arms producing noisier data. \textbf{(2) Data integrity and privacy.} For example, when data is gathered through surveys, topical bias~\cite{paulus2023reinforcing} can render significant phenomena invisible in the available data due to certain survey sections being rejected by authorities or dismissed by the impacted populations. Additionally, driven by the principle of differential privacy, noise might be intentionally added to the data~\cite{dwork2014algorithmic}.


Motivated by these scenarios, in this paper we study the RMAB model where some arms are affected by noise in their observed rewards at some states, with these noisy arms and rewards not known a priori. The challenge of applying existing RL methods to this setting is that
%, when trained exclusively on noisy reward data, 
systematic errors might create false optima, preventing the exploration of states with true high rewards and leading to suboptimal actions selected by the RMAB. For example, the aforementioned systematic overestimation errors of women's delivery dates can lead to suboptimal resource allocation, thereby reducing the number of deliveries in healthcare facilities~\cite{fulcher2020errors}. %Exploration may allow us to reach a true high-reward state where there are a large number of deliveries in healthcare facilities.

% We further explore how to conduct effective RMAB learning despite the existence of systematic reward errors. The idea is to allow the arms to learn to communicate useful information with each other that helps learn more accurate local Q functions. In our framework, each arm has a binary communication action. Opting to communicate enables an arm to receive the local Q function parameters of a similar arm as the message. Using these parameters, the receiver arm establishes a behavior policy that guides the collection of experience samples that are used in an attempted local Q function update. This behavior policy may help escape the false optima.
%e.g., communication may allow women to estimate the delivery dates more accurately, leading to appropriate resource allocation and improved health facility deliveries~\cite{fulcher2020errors}.

% Intuitively, if local Q updates under communication can lead to a higher return for the RMAB, we can encourage and reinforce the corresponding communication actions. Therefore, we adopt Q-learning for communication learning with the communication reward calculated as the difference in the RMAB return with and without communication. However, this communication reward captures the joint influence of communication actions of all arms. To deal with the credit assignment problem here, we adopt a decomposed Q network architecture, through which the joint communication Q function is factorized into local communication Q functions. %In this way, the arms can make communication decisions based on local information post-deployment.

%We further explore effective RMAB learning despite systematic reward errors by enabling arms to learn to communicate useful information to improve local Q-learning
We propose the first communication learning approach in RMABs 
to deal with systematic reward errors, enabling arms to learn to communicate useful information to improve local Q-learning. We formally model the communication learning problem as a Multi-Agent MDP~\cite{boutilier1996planning}, which is in addition to and distinct from per-arm MDP without considering communication. In this framework, each arm has a binary communication action. Choosing to communicate allows an arm to receive the local Q function parameters from a similar arm. Using these parameters, the receiving arm establishes a behavior policy to collect experience samples for updating its local Q function. This behavior policy may enable exploration and help escape false optima. In this way, the communication reward can be calculated as the difference in RMAB return with and without communication. We then adopt Q-learning for communication learning. Since RMABs optimize a centralized objective involving return from all the arms, the communication reward captures the joint influence of communication of all arms.
%However, due to the existence of a central planner, we can only get a communication reward that captures the joint influence of the communication actions of all arms. 
To solve this problem and learn the individual communication strategy of each arm, we propose to use a decomposed Q-network architecture for communication learning that factorizes the joint communication Q function into local communication Q function.
%To address the credit assignment problem, we use a decomposed Q network architecture to factorize the joint communication Q function into local communication Q functions.

% To demonstrate the effectiveness our method, we formally model the communication learning problem as a Multi-Agent MDP~\cite{boutilier1996planning} and rigorously compare the sample complexity required to learn a near-optimal Q function when learning with and without communication. 
To demonstrate the effectiveness our method, we rigorously compare the sample complexity required to learn a near-optimal per-arm Q function when learning with and without communication. 
We show theoretically that there exists RMABs where communication from non-noisy to noisy arms can reduce the Q estimation errors exponentially with respect to the number of states. 
Interestingly, further studies reveal that communication from noisy to non-noisy arms can also be beneficial, provided that the behavior policy, on the receiver arms' MDP, achieves reasonable coverage over the state-action space and does not decorrelate too slowly from the initial states.

Empirically, we validate our method on synthetic problems, as well as the ARMMAN maternal healthcare~\cite{vermagroup} and the SIS epidemic intervention problem~\cite{yaesoubi2011generalized} built upon real-world data. Results show that our method significantly outperforms both the non-communicative learning approach and the approach with fixed communication strategies, achieving performance levels comparable to those learning in noise-free environments. Results are robust across problems, resources budgets, and noise levels. Furthermore, visualization of the learned communication strategies supports our theoretical findings that communication from noisy arms to non-noisy arms, and vice versa, can be helpful.


% we conduct a rigorous comparison of the sample complexity required to learn a near-optimal Q function through learning with and without communicationThis analysis helps establish conditions under which communication proves beneficial.  In particular, we find that the influence of communication closely dependent on the coverage rate and mixing time~\cite{hsu2015mixing} of the behavior policy in the receiver MDP.
%Communication has also been studied in the context of distributed (PO)MDPs~\cite{kwak2010teamwork,nair2004communications,tasaki2010introducing}. 

\textbf{Related works}.\ To the best of our knowledge, this is the first work that introduces communication into RMABs. This is perhaps surprising given that communication is an important topic that has been extensively studied in other multi-agent problems. In Dec-POMDPs~\cite{oliehoek2016concise,kwak2010teamwork,nair2004communications}, previous works explore decentralized communication learning~\cite{sukhbaatar2016learning,hoshen2017vain, jiang2018learning, singh2019learning,wang2019learning}, the emergence of natural language~\cite{foerster2016learning,das2017learning,lazaridou2017multi, mordatch2018emergence,zhao2024ai4sg,kang2020incorporating}, and implicit communication by coordination graphs~\cite{bohmer2020deep,wang2021context,kang2022non,yang2022self}, influence on each other~\cite{jaques2019social,wang2019influence}, and attention mechanisms~\cite{huang2020one,kurin2020my,dong2022low,dong2023symmetry}. Different from these works, we consider communication under noisy returns and in the RMAB setting where the central planner policy constrained by resource budgets determines the influence of communication. 

In the literature of cooperative multi-agent reinforcement learning~\cite{yu2022surprising,wen2022multi,kuba2021trust,wang2020roma,christianos2020shared,peng2021facmac,wang2020dop,jiang2019graph,wang2020rode,nagaraj2023multi}, value decomposition methods~\cite{sunehag2018value,rashid2018qmix,son2019qtran,li2021celebrating} have recently witnessed great success in addressing challenges such as partial observability and learning scalability. 
These methods decompose the joint Q-value conditioned on true states and joint actions into per agent local Q functions based on local action-observation history and local actions. 
% In these methods, each agent has a local Q function based on local action-observation history and local actions. The joint Q value conditioned on true states and joint actions is learned to be a combination of local Q values. 
In this work, we adopt a linear value decomposition framework~\cite{sunehag2018value} for the communication Q network to solve the unique problems of learning with the presence of noisy arms.
% Furthermore, in this paper, we develop communication , which existing works fail to address. 


==> text/2-Preliminary.tex <==
\section{Preliminaries}

\subsection{RMABs with Noisy Arms}

We study multi-action Restless Multi-Arm Bandits (RMABs) with $N$ arms. Each arm $i\in[N]$ is associated with a Markov Decision Process $\mathcal{M}_i=(\mathcal{S}_i, \mathcal{A}_i, \mathcal{C}_i, T_i, R_i,\beta, \bm z_i)$. Here, $\mathcal{S}_i$ is the state space that can be either discrete or continuous. The reward at a state is given by a function $R_i: \mathcal{S}_i \rightarrow\mathbb{R}$, and $\beta\in[0,1)$ is a discount factor for future rewards. We assume that there is a set of \textbf{noisy arms} $\mathcal{N}_\epsilon\subset [N]$, and the rewards of a noisy arm $i\in \mathcal{N}_\epsilon$ are unreliable and affected by noise $\epsilon_i(s_i)$ at some states $s_i\in\mathcal{S}_{\epsilon,i}\subset\mathcal{S}_{i}$. We consider systematic errors: $\tilde{R}_i(s_i) = R_i(s_i)+\epsilon_i(s_i)$, where $\epsilon_i(s_i)$ is sampled from a distribution $\mathcal{E}_i$ and fixed during training and testing. The identity of noisy arms $\mathcal{N}_\epsilon$, the affected states $\mathcal{S}_{\epsilon,i}$, the reward noise $\epsilon_i$, and its distribution $\mathcal{E}_i$ are not known a priori.

$\mathcal{A}_i$ is a finite set of discrete actions. Each action $a\in\mathcal{A}_i$ has a cost $\mathcal{C}_i(a)$. Following the standard bandit assumption that an arm can be "not pulled" at no cost, we set $\mathcal{C}_i(0)=0$. The probability of transitioning from one state to another given an action is specified by the function $T_i: \mathcal{S}_i\times \mathcal{A}_i \times \mathcal{S}_i \rightarrow[0,1]$. In line with previous work~\cite{zhao2023towards,elmachtoub2023estimate,zhao2022implicit,elmachtoub2023balanced}, we assume that $\mathcal{S}_i, \mathcal{A}_i$, and $\mathcal{C}_i$ are the same for all arms $i\in[N]$ and omit the subscript $i$ for simplicity. Each arm has a feature vector $\bm z_i\in\mathbb{R}^m$ that provides useful information about the transition dynamics of arm $i$. We define the arm with the most similar features with arm $i$ as $\nu_i=\arg\min_j\|z_j-z_i\|_2$.

% \tw{Closest feature and transition?}

We consider a constrained global resource setting where, at every timestep $t\in[H]$, where $H$ is the horizon, the total cost of actions taken is no greater than a given budget $B$. Under this constraint, the \emph{central planner} selects one action for each of the $N$ arms at each timestep. Formally, the central planner has a policy $\pi$ to maximize its expected discounted return $G(\pi) = \mathbb{E}_\pi[\sum_{t=1}^H \beta^t\sum_{i\in[N]}R_i(s_i^t)]$, where $s_i^t$ is the state of arm $i$ at time step $t$. $\pi$ is typically computed by solving the constrained Bellman equation~\cite{hawkins2003langrangian,killian2021beyond,killian2022restless}:
\begin{align}
\label{eq:original_opti_problem}
&J(\boldsymbol{s})=\sum_{i=1}^N R_i\left(s_i\right)+\beta \, \max _{\boldsymbol{a}}\mathbb{E}_{\boldsymbol{s}^{\prime}}\left[J\left(\boldsymbol{s}^{\prime}\right) \mid \boldsymbol{s},\boldsymbol{a}\right] \nonumber\\
&\text { s.t. } \sum_{i=1}^N \mathcal{C}(a_i)\leq B .
\end{align}
% &\text { s.t. } \sum_{i=1}^N \sum_{j=1}^{|\mathcal{A}|} \boldsymbol{A}_{i j} c_j \leq B \quad \text{and} \quad \sum_{j=1}^{|\mathcal{A}|} \boldsymbol{A}_{i j}=1 \quad \forall i \in[N]\, ,\nonumber
% where $c_j = \mathcal{C}(a_j)$ is the cost of $j^{\text{th}}$ action. $\bm A\in\{0,1\}^{N\times |\mathcal{A}|}$ denotes one-hot-encoding of the actions taken over all arms. $A_{ij} = 1$ if action $j$ is chosen by arm $i$ and $A_{ij} = 0$ otherwise.

\subsection{Reinforcement Learning in RMABs}

Deep reinforcement learning has been proven to be efficient in solving the RMAB problem~\cite{avrachenkov2022whittle,killian2022restless,zhao2024towards}. To learn arm policies, we take the Lagrangian relaxation of the budget constraint~\cite{hawkins2003langrangian}, defining
\begin{align}
    J(s,\lambda) = \frac{\lambda B}{1-\beta}+\sum_{i=1}^N \max_{j\in[A]}\left\{Q_i(s_i,j)\right\},
\end{align}
where $Q_i$ is arm $i$'s Q function estimating its expected discount return of an action at a state. We use deep Q-learning
and parameterize the action-value function $Q_i(s_i, a_i; \theta_i)$ of each arm $i$ with $\theta_i$, which is updated by the TD-loss \cite{sutton2018reinforcement,killian2021beyond}:
\begin{align}\label{equ:q_td_loss}
\mathcal{L}_\texttt{TD}(\theta_i) =& \mathbb{E}_{(s_i, a_i, s_i')\sim\mathcal{D}}\Big[\Big(R_i(s_i)-\lambda \mathcal{C}(a_i)\nonumber\\ 
&+ \beta \max_a Q_i(s_i',a;\theta_i)-Q_i(s_i,a_i;\tilde{\theta}_i)\Big)^2\Big],
\end{align}
where $Q_i(\cdot;\tilde\theta_i)$ is a target network whose parameters are periodically copied from $Q_i$. The expectation means that the samples come from a replay buffer $\mathcal{D}$.

% To recover a planner policy that respects the budget constraint, previous work construct a knapsack problem with $Q_i(s_i, a_i)$ as values, $\mathcal{C}_i(s_i)$ as weights, and the constraints in the optimization problem~\ref{eq:original_opti_problem}. The knapsack solution finds the joint action with largest sum of the learned $Q_i$ values conform to the budget constraint.

To \textit{infer} a central planner policy that adheres to the budget constraint, previous research~\cite{killian2022restless} constructs a knapsack problem using $Q_i(s_i, a_i)$ as values and $\mathcal{C}(a_i)$ as weights, within the constraints defined in the optimization problem \ref{eq:original_opti_problem}. The solution to this knapsack problem identifies the joint action that maximizes the sum of the learned $Q_i$ values while conforming to the budget constraint. In this case, we denote the planner policy by $\pi(\bm\theta)$ to highlight its dependency on the joint parameters of individual Q-functions $\bm\theta=(\theta_1,\cdots,\theta_N)$.

% For an actor-critic methods, after performing an update of the Q-function in the critic, one may compute the advantage estimate: % \cite{konda1999actor}:
% $$
% A\left(\mathbf{s}, \mathbf{a}\right)=Q\left(\mathbf{s}, \mathbf{a}\right)-V\left(\mathbf{s}\right).
% $$ 
% % $$
% % A^{\pi}\left(\mathbf{s}, \mathbf{a}\right)=Q^{\pi}\left(\mathbf{s}, \mathbf{a}\right)-V^{\pi}\left(\mathbf{s}\right).
% % $$ 
% In practice, the values $A(s,a), Q(s,a), V(s)$ will be evaluated based on the current policy $\pi$. Intuitively, the advantage estimate tells us how much better $\mathbf{a}$ is compared to the current policy $\pi$. The advantage estimate is then plugged into the policy gradient to update the actor.

% To learn an action charge $\lambda$, we follow an updating rule \cite{killian2022restless}:
% \begin{align*}
% \Lambda_t \leftarrow& \Lambda_{t-1} - \alpha_{\Lambda}\left(\frac{B}{1-\beta} +\sum_{n=1}^N\sum_{t=0}^H\mathbb{E} \beta^t c_{n,t}\right),
% \end{align*}
% where $c_{n,t}$ is the cost of the
% action taken by the optimal policy on arm $n$ in round $t$, and $\alpha_{\Lambda}$ is the step size.  


% \subsection{Value Decomposition}

% In the literature of cooperative multi-agent reinforcement learning, value decomposition methods have recently witnessed great success in learning cooperative policies in partial observable environments. In these methods, each agent has a local Q function $Q_i(\tau_i,a_i)$ based on local action-observation history $\tau_i$. The joint Q function $Q_{tot}(\bm\tau,\bm a)$ is conditioned on the joint 

% In our work, we use value decomposition methods for communication learning. 

% extend the  to support distributional Q-functions to deal with the noisy rewards in arms.

==> text/3-Methods.tex <==
\section{RMAB Learning with Communication}

In this section, we introduce our method of learning communication to share useful knowledge among arms. We first define the communication problem as a Multi-Agent MDP~\cite{boutilier1996planning} and address the following problems: (1) What are 
the messages? (Sec.~\ref{sec:method:comm_problem}) How do they affect local Q learning? (Sec.~\ref{sec:method:comm_dynamics}) (2) How to generate reward signals that measure the influence of communication? (Sec.~\ref{sec:method:comm_reward}) (3) How to use the communication reward to learn communication strategies? (Sec.~\ref{sec:method:comm_decomposed}) (4) Why and under what conditions can communication help learning? (Sec.~\ref{sec:method:comm_dynamics} and~\ref{sec:theory})

% (4) Robustness design: how to deal with the influence of random rewards in each arm on communication learning? In Sec.~\ref{sec:alg_com}, we answer these four questions and describe the details of communication learning. In Sec.~\ref{sec:alg_all}, we describe the overall RMAB learning with communication algorithm, addressing the problem of how to interleave communication learning and policy learning for each arm.

\subsection{Define the Communication Learning Problem}\label{sec:method:comm_problem}

Akin to traditional deep RMAB learning algorithms~\cite{fu2019towards,biswas2021learn,killian2022restless,avrachenkov2022whittle}, our approach involves each arm learning its local Q networks $Q_i(s_i, a_i; \theta_i)$ to predict the expected return of taking action $a_i$ in state $s_i$. The central planner then selects centralized actions based on the local Q values.

When the data source is noisy, the local Q functions may be inaccurate, leading to the central planner choosing suboptimal actions. Figure~\ref{fig:r2u_helpful} in Appendix~\ref{appx:proof:examples} shows such an example. To address this issue, we introduce a mechanism that allows each arm to learn a communication policy that diminishes the impact of noisy data and enhances the overall effectiveness of the central planner.

We define the communication learning problem within the framework of a Multi-Agent MDP~\cite{boutilier1996planning}.
\begin{definition}[The Communication MDP]
    The communication MDP in the RMAB setting is modelled by a multi-agent MDP $\mathcal{M}^\texttt{c}=(\mathcal{S}^\texttt{c}, I, \mathcal{A}^\texttt{c}, T^\texttt{c}, \comr)$. $I$ is the set of players, which in our case is the set of arms. $\mathcal{S}^\texttt{c}=\Theta$ is the state space, where $\Theta$ is the joint parameter space of Q networks. $\bm\theta=(\theta_1,\cdots,\theta_N)\in \mathcal{S}^\texttt{c}$ corresponds to joint Q function parameters. $\mathcal{A}^\texttt{c}=\{0,1\}^I$ is the action space. $\coma{i}=1$ means arm $i$ decides to ask Q network parameters from the arm with the most similar features, $\nu_i$, as the message. If $\coma{i}=0$, arm $i$ will not receive a message. The joint communication action $\jcoma$ leads to a transition in $\bm\theta$ (Eq.\ref{equ:coms_t}) and a reward $\comr$ (Eq.~\ref{equ:comm_r}).
\end{definition}
% \dn{ An MDP requires the following things to be completely defined completely. Currently, these things are spread out over the sections. If we can either define them at one place or reference where they are defined, it would be helpful:
% \begin{enumerate}
%     \item State space
%     \item Action Space
%     \item Reward for a given state and action
%     \item state evolution given action.
% \end{enumerate}
% Some more comments:
% In the Definition above, explicitly define $\mathcal{S}^{\texttt{c}} = \Theta^{I}$ where $\Theta$ is the parameter space of a single Q network. That is, $\bm\theta = (\theta_1,\dots,\theta_N) \in \mathcal{S}^{\texttt{c}}$ where $\theta_i$ corresponds to the current Q-function parameter of arm $i$.
%   $\mathcal{A}^{\texttt{c}} = \{0,1\}^{I}$. The action $(a^{\texttt{c}}_1,\dots,a_N^{\texttt{c}}) \in \mathcal{A}^{\texttt{c}}$ is such that $a^{\texttt{c}}_{i} = 1$ means arm $i$ decides to obtain Q-value parameters from its nearest arm $\nu_i$.   }
The definition of this Communication MDP is associated with the underlying RMAB in the sense that the Communication MDP solution affects the action selection of the central planner. After every $K$ learning epochs of $Q_i$ in the MDP $\mathcal{M}_i$, parameters of arms' Q functions are used as the state for this Communication MDP $\mathcal{M}^\texttt{c}$. We assume that each arm $i$ in the system has the chance to communicate with the arm with the most similar features, denoted by arm $\senderfor{i}$. This results in $N$ possible communication channels (i.e. arm $i$ will receive a message if $\coma{i}=1$). In this way, the set of players in $\mathcal{M}^\texttt{c}$ is the set of arms $[N]$. In addition to selecting actions in the arm MDP $\mathcal{M}_i$, each arm also selects actions in this Communication MDP $\mathcal{M}^\texttt{c}$. These \emph{communication actions} determine the communication channel activation pattern, which remains frozen for the next $K$ learning epochs. We will discuss the details in the following subsections.

An alternative design option is to adopt a denser communication scheme, \ie, an arm can receive messages from multiple other arms. As formally detailed in Proposition~\ref{prop:sparse_com} in Sec.~\ref{sec:theory}, under certain assumptions regarding concentratability~\cite{munos2003error,chen2019information}, our sparse communication scheme is shown to effectively learn near-optimal value functions with the same errors as the dense scheme. Therefore, we favor the sparse scheme due to its lower demands on communication bandwidth.

% both sparse and dense communication schemes can learn . Additionally, we demonstrate that the difference in sample complexity required to achieve this grows at most linearly with the number of senders to each arm.

\subsection{Communication Actions and Transition Dynamics}\label{sec:method:comm_dynamics}
We now describe how the communication action $\jcoma$ induces a state transition in the space $\mathcal{S}^\texttt{c}$. Specifically, when $\coma{i}$ is 1, arm $i$ receives a message from arm $\senderfor{i}$, which is the parameters of the local Q network of arm $\senderfor{i}$, $\theta_{\nu_i}$. Using this message, arm $i$ formulates a behavior policy $\pi_{{\senderfor{i}}}$ as follows:
\begin{align}
    \pi_{{\senderfor{i}}}(\cdot|s_i)=\texttt{SoftMax}\left(Q_{\senderfor{i}}(s_i,\cdot)\right).
\end{align}
Using behavior policy $\pi_{{\senderfor{i}}}$, arm $i$ navigates in its arm MDP $\mathcal{M}_i$, collecting transition samples in a replay buffer $\mathcal{D}_{\pi_{\senderfor{i}}}$. This buffer is then used to update the local Q-network. Therefore, the TD-loss for arm $i$ with the communication channel $i$ activated is given by:
\begin{align}
\mathcal{L}^\texttt{c}_\texttt{TD}(\theta_i|\coma{i}\shorte 1) = & \mathbb{E}_{(s_i, a_i, s_i')\sim\mathcal{D}_{\pi_{\senderfor{i}}}}\Big[\Big(R_i(s_i)-\lambda c_{a_i} \nonumber\\
&+ \beta \max_a Q_i(s_i',a;\theta_i)-Q_i(s_i,a_i;\tilde{\theta}_i)\Big)^2\Big].\nonumber
\end{align}

Alternatively, if arm $i$ opts not to receive communication, it engages in the $\epsilon$-greedy strategy to explore the MDP $\mathcal{M}_i$ and generate the replay buffer. Therefore, 
\begin{align}
    \mathcal{L}^\texttt{c}_\texttt{TD}(\theta_i|\coma{i}\shorte 0)=\mathcal{L}_\texttt{TD}(\theta_i).
\end{align}
As such, the updates to local Q parameters are dependent on the communication action:
\begin{align}
    \theta_i'(\coma{i}) = \theta_i - \alpha\nabla_{\theta_i}\mathcal{L}^\texttt{c}_\texttt{TD}(\theta_i|\coma{i}),\label{equ:coms_t}
\end{align}
where $\alpha$ is the learning rate. Eq.~\ref{equ:coms_t} specifies the state transition dynamics of the Communication MDP.

% If multiple messages are received by arm $j$, we use their average:
% \begin{align}
% \mathcal{L}^\texttt{c}_\texttt{TD}(\theta_j|\jcoma) = \mathbb{E}_{(s_j, a_j, s_j')\sim\mathcal{D}}\left[\left(R(s_j)-\lambda c_{a_j} + \beta \max_a \sum_{i:\coma{i}{j}=1}Q(s_j',a;\theta_i)-Q_j(s_j,a_j;\theta_j)\right)^2\right].
% \end{align}
% where $\jcoma$ is the joint communication action consisting of all $\coma{i}{j}$. 

\subsection{Communication Reward}\label{sec:method:comm_reward}
% Intuitively, communication from a noisy arm to a non-noisy arm may appear advantageous, as it allows for the collection of learning samples via a behavior policy free from reward noise. This concept is supported in Lemma~\ref{lemma:r2u_useful} (Sec.~\ref{sec:theory}), which demonstrates that there exists a family of RMABs where, without communication, a noisy arm can exhibit an exponential Q-value error in the number of states, even after a number of learning epochs also exponential in number of states. However, such communication is not always beneficial. Lemma~\ref{lemma:r2u_useless} (Sec.~\ref{sec:theory}) reveals that another scenario with a family of RMABs where such communication leads to an exponential higher sample complexity for learning a near-optimal Q function in the noisy arm, especially when the arm MDPs are dissimilar.

% To analyze these seemingly contradictory observations and to thoroughly investigate the influence of communication on the Q-learning in the receiver arm, we rigorously compare the sample complexity of learning a near-optimal Q function with and without communication in Proposition~\ref{prop:utor} of Sec.~\ref{sec:theory}. We discover that, for communication to enhance Q-learning sample complexity, we expect two properties of the behavior policy $\pi_{\nu_i}$ on the receiver MDP $\mathcal{M}_i$: (1) $\pi_{\nu_i}$ achieves a reasonable coverage of the state-action space; (2) $\pi_{\nu_i}$ does not decorrelate from the initial states too slowly. Please see Proposition~\ref{prop:utor} for more details. Notably, this conclusion is applicable across different sender-receiver types, allowing for both the sender and receiver arms to be either noisy or non-noisy. 

Lemma~\ref{lemma:r2u_useful} and~\ref{lemma:r2u_useless} in Sec.~\ref{sec:theory} reveal that some seemingly reasonable fixed communication patterns, 
%like those from a noisy arm to a non-noisy arm, 
like those from a non-noisy arm to a noisy arm, 
can lead to an exponential higher sample complexity for learning a near-optimal Q function in the noisy arm. In fact, as shown in Proposition~\ref{prop:utor} of Sec.~\ref{sec:theory}, the influence of communication is determined by the state-action space coverage and the mixing time of the behavior policy $\pi_{\nu_i}$ on the receiver arms.

% Under certain conditions, seemingly intuitive communications pattern do not effectively address the issue of data unreliability. % To decide whether arm $i$ should communicate with arm $j$, we need to estimate the utility of the activation of this communication channel, which is measured by a channel-level communication Q-function $\comQ{i}{j}$. 

These findings highlight the intricate and dynamic nature of the communication learning problem in RMAB. In practice, to adaptively decide the optimal communication action, we propose that each arm learns a communication Q function $\comQ{i}$. This approach encounters obstacles in the RMAB setting, where clear, separate reward signals for each $\comQ{i}$ are absent. The central planner policy instead bases action decisions on the updated Q-functions of all arms and the budget. The collaborative contribution of the joint communication action $\jcoma$ to the learning objective is:
\begin{align}\label{equ:comm_r}
    \comr(\bm\theta,\jcoma) = G_T\left(\pi(\bm\theta'(\jcoma))\right) - G_T\left(\pi(\bm\theta'(\bm 0))\right).
\end{align}
Here, $G_T(\pi) = \frac{1}{T}\sum_{k=1}^T[\sum_{t=1}^H \beta^t\sum_{i\in[N]}R_i(s_i^{k,t})]$ is the empirical return under policy $\pi$ averaged over $T$ episodes,
% \begin{align}
%     G_T(\pi) = \frac{1}{T}\sum_{k=1}^T\left[\sum_{t=1}^H \beta^t\sum_{i\in[N]}R_i(s_i^{k,t})\right],
% \end{align}
where $s_i^{k,t}$ is arm $i$ state at timestep $t$ of episode $k$. $\pi(\bm\theta'(\jcoma))$ and $\pi(\bm\theta'(\bm 0))$ are the planner policies with the arm Q-functions updated with and without messages, respectively. The communication reward is defined as the difference in the planner's return in these two cases.



\subsection{Decomposed Communication Q Function}\label{sec:method:comm_decomposed}
With the definition of the communication reward (Eq.~\ref{equ:comm_r}), the simplest strategy of communication learning is to estimate a \emph{joint} communication action-value function $\jcomQ(\bm\theta, \jcoma)$. However, the question is that there are $N$ communication channels, and even though our communication action is binary, there are $O(2^{N})$ possible joint actions $\jcoma$. With this exponential number of actions, it is challenging to conduct deep Q-learning, which requires a maximization operation over the whole action space.



We propose to solve this problem by value decomposition~\cite{sunehag2018value}. Specifically, we represent the global communication Q-function as a summation of the channel-level, individual communication Q-functions:
\begin{align}\label{equ:decomp}
    \jcomQ(\bm\theta, \jcoma;\bm\xi) = \sum\nolimits_{i\in[N]}\comQ{i}(\bm\theta, \coma{i};\xi_{i}).
\end{align}
Here, $\xi_{i}$ is the parameters of the channel-level communication Q-function, and $\bm\xi$ is the joint parameter consisting of all $\xi_{i}$. Such a decomposition satisfies an important property:
\begin{align}
    \arg\max_{\jcoma} \jcomQ = \left(\arg\max_{\coma{1}}\comQ{1},\cdots,\arg\max_{\coma{N}}\comQ{N}\right),
\end{align}
which is because Eq.~\ref{equ:decomp} allows $\partial\jcomQ/\partial \comQ{i}\ge 0$. This means that the joint action that maximizes the $\jcomQ$ can be obtained by independently selecting the local communication action that maximize $Q_i$. As a whole, network $\jcomQ(\cdot;\bm\xi)$ is a standard Q-network conditioned on states $\bm\theta$ and actions $\jcoma$, allowing it to be trained using joint rewards $\comr$ (Eq.~\ref{equ:comm_r}). On a finer level, it has a decomposable structure simplifying the $\arg\max$ calculation. Therefore, $\jcomQ(\cdot;\bm\xi)$ can be trained by the following TD-loss:
\begin{align}
&\mathcal{L}^\texttt{d}_\texttt{TD}(\bm\xi) = \mathbb{E}_{(\bm\theta,\jcoma,\bm\theta')\sim\mathcal{D}}\Big[\Big(\comr(\bm\theta,\jcoma)  \nonumber\\
& +\beta \sum\nolimits_{i\in[N]}\max_{a} \comQ{i}(\bm\theta', a; \tilde{\xi}_i)-\sum\nolimits_{i\in[N]}\comQ{i}(\bm\theta, \coma{i};\xi_{i})\Big)^2\Big].\nonumber
\end{align}
$\comQ{i}(\cdot; \tilde{\xi}_i)$ is a target network with parameters periodically copied from $\comQ{i}$, and $\mathcal{D}$ is a replay buffer. In this way, we implicitly achieve credit assignment, because we use a joint reward $\comr$ for training but get a set of Q functions for individual arms, which can recover the best joint action locally.

% Therefore, during the inference time, the communication strategy of each arm $i$ can be established by selecting $\coma{i}=\arg\max_{\coma{i}} \comQ{i}$.



% \textbf{Dealing with noise}.\ \ [Change the communication Q function to distributional. Prove that it still conforms to IGM. Write this after obtaining experimental results.]

% 
% % \subsection{Overall Learning Framework}~\label{sec:alg_all}

==> text/3.1-Theory.tex <==
 \section{Theoretical Analysis}\label{sec:theory}
We begin by investigating the influence of communication and establishing the specific conditions under which communication can reduce the sample complexity for the receiver arm in learning a near-optimal Q function. We define the minimum state-action occupancy probability,
\begin{align}
    \mu_{\texttt{min}} := \min_{s,a}\mu_{\pi_{\nu_i}}(s,a),
\end{align}
as the lowest probability of any state-action pair under the stationary distribution $\mu_{\pi_{\nu_i}}$ induced by the behavior policy $\pi_{\nu_i}$ on the receiver MDP, where $\nu_i$ is the arm with the most similar feature to arm $i$. We further define the mixing time~\cite{hsu2015mixing,li2020sample},
\begin{align}
    t_\texttt{mix} = \min\left\{t|\max_{s_0,a_0}\sup_{s,a} |P^t(s,a|s_0,a_0)-\mu_{\pi_{\nu_i}}(s,a)|\le\frac{1}{4}\right\},
\end{align}
where $P^t$ is the state-action distribution at timestep $t$ given the initial state and action. The mixing time $t_\texttt{mix}$ captures how fast the behavior policy decorrelates from the initial state. We now show the condition under which communication can be helpful.

\begin{restatable}[Useful Communication]{proposition}{usefulcom}\label{prop:utor}
For the Q-learning of arm $i$, when
\begin{align}
    \mu_{\texttt{min}}>\frac{2(1-\beta)^2}{|\mathcal{S}||\mathcal{A}|},\ \ \text{and}\ \ t_\texttt{mix}\le \frac{1}{\epsilon_e^2(1-\beta)^4},
\end{align}
with a probability at least $(1-\delta)^2$ for any $0<\delta<1$, compared to learning without communication, choosing to receive communication and using behavior policy $\pi_{\nu_i}$ leads to better sample complexity in the worst case for learning $\epsilon_e$-optimal Q function such that $\|Q_i(s,a)-Q_i^*(s,a)\|<\epsilon_e, \forall (s,a)$.
\end{restatable}

The Proof is detailed in Appendix~\ref{appx:proof:useful_com}. Proposition~\ref{prop:utor} shows that communication can accelerate arm $i$'s Q-learning as long as $\pi_{\nu_i}$ visits every state-action pair with a small probability and is not too slowly disentangling from the initial state. This finding is solely dependent upon the characteristics of the behavior policy in the receiver MDP $\mathcal{M}_i$ and does not require the sender or the receiver to be non-noisy or noisy.

We then analyze the effectiveness of a sparse communication strategy. Specifically, we compare our setup where each arm $i$ receives messages from an arm $\nu_i$ against a dense communication scheme where arm $i$ receives messages from $d$ other arms. In the dense communication scheme, the behavior policy $\pi_{\bar{\nu}_i}$ is the average of policies from all senders. Specifically, we collect the same number of samples using each sender's policy and amalgamate them into a unified experience replay buffer.


% \dn{Average here could mean two things: the policy given state is the average of the policies or we obtain a mixture of the trajectories. Proposition 4 works when we have the former. Can you clarify?}

The following assumption on concentratability asserts that both $\pi_{\nu_i}$ and $\pi_{\bar{\nu}_i}$ provide a reasonable coverage over the state-action space.
\begin{assumption}[Concentratability Coefficient]
There exists $C_{\nu_i}<\infty$, $C_{\bar{\nu}_i}<\infty$ s.t.
\begin{align}
    \frac{v(s,a)}{\mu_{\bar{\nu}_i}(s,a)}\le C_{\bar{\nu}_i} \text{ and } \frac{v(s,a)}{\mu_{\nu_i}(s,a)}\le C_{\nu_i} \text{, for } \forall(s,a)\in(\mathcal{S}, \mathcal{A}),\nonumber
\end{align}
for any admissible distribution $v$ that can be generated by following some policy for some timesteps in the MDP $\mathcal{M}_i$. Here $\mu_{\nu_i}$ and $\mu_{\bar{\nu}_i}$ are the stationary distribution of $\pi_{\nu_i}$ and $\pi_{\bar{\nu}_i}$ on $\mathcal{M}_i$, respectively.
\end{assumption}
Under this assumption, we can prove that the sparse communication scheme can also learn a near-optimal Q function as under the dense scheme. The key observation that underpins the proof is $\frac{1}{d}\mu_{\nu_i}(s,a)\le \mu_{\bar{\nu}_i}(s,a)$, where $d<N$ is the maximum number of other arms that can send messages to arm $i$. The convergence of the communication learning under the dense scheme implies that $C_{\bar{\nu}_i}$ is finite, which further indicates the finiteness of $C_{\nu_i}$ and thus the convergence of the communication learning of the sparse scheme.
\begin{restatable}[Sparse Communication]{proposition}{sparsecom}\label{prop:sparse_com}
For a dense communication strategy, there exists a sparse communication strategy which approximates the optimization step in Equation~\eqref{equ:coms_t} faithfully. Additionally, both these two strategies can learn near-optimal value functions, and the sparse communication scheme requires at most $O(d)$ times more samples to achieve this.
\end{restatable}

Detailed proof is deferred to Appendix~\ref{appx:proof:sparse_com}. We next show that a communication channel from a non-noisy arm to a noisy arm can be either helpful (Lemma~\ref{lemma:r2u_useful}) or detrimental (Lemma~\ref{lemma:r2u_useless}), depending on the specific structures of the sender and receiver MDPs.

% The intuition is that communication proves advantageous when the arm MDPs exhibit similarity.

\begin{restatable}{lemma}{ruuseful}\label{lemma:r2u_useful}
    There exists a family of RMABs where, without communication from non-noisy arms to noisy arms, the error in Q values of a noisy arm could be $\max_{s,a}|Q_i^*(s,a)-Q_i(s,a)|=O\left((\frac{1}{\beta})^{|\mathcal{S}|}\right)$ even after $O\left((\frac{1}{\epsilon})^{|\mathcal{S}|}\right)$ epochs. $\epsilon\in(0,1)$ is the exploration rate in $\epsilon$-greedy exploration scheme. By contrast, this Q error can be reduced to 0 with communication from non-noisy arms to noisy arms.
\end{restatable}

\begin{restatable}{lemma}{ruuseless}\label{lemma:r2u_useless}
    There exists a family of RMABs where, with communication from a non-noisy arm to a noisy arm, we need $O\left((\frac{1}{\epsilon})^{|\mathcal{S}|}\right)$ times more samples to learn a near-optimal Q function in the noisy arm than without communication.
\end{restatable}

The proofs of Lemma~\ref{lemma:r2u_useful} and~\ref{lemma:r2u_useless} can be found in Appendix~\ref{appx:proof:examples}. The observation that the errors in the Q function and the sample complexity of Q learning can increase exponentially with the number of states in the worst case scenarios highlights the need to move away from predefined communication channels. Instead, communication Q-learning provides a more adaptable and effective approach.

==> text/4-Experiments.tex <==
%Inspired by the vast literature on agent-based epidemic modeling \cite{kerr2021covasim,hinch2021openabm}

\section{Experiments}
\begin{figure*}[t]
\includegraphics[width=\textwidth]{figs/main_results_figure.pdf}
        \caption{Performance (interquartile mean \cite{agarwal2021deep} and standard error of return over 200 random seeds) of our method, baselines, and ablations in three environments with different numbers of arms $N$ and resource budgets $B$. Communication learning starts at epoch 200. We present results on \textbf{two additional baseline} in Tables~\ref{table:noise_level_ablation} and \ref{table:num_noisy_arms_ablation} (see Appendix\ref{appx:exp_details} for more ablations).}
        \label{fig:main_result_figure}
\end{figure*}

We present experimental evaluations and ablation studies to investigate: (1) The learning performance of our communication method compared to baselines; (2) The characteristics of learnt communication strategies; (3) The robustness of our method in terms of resource budgets, the number of arms, noise types and levels. We discuss additional experimental details and hyperparameters in Appendix~\ref{appx:exp_details}. 

% \textbf{Experiment Setup.}\ \ We evaluate our methods on the following domains.
% a synthetic setting, an epidemic modeling scenario, and a maternal healthcare intervention task, each designed to test the efficacy of our model under different conditions. Noisy arms observe rewards drawn from a perturbed reward function $\tilde{R}(s) = R(s)+\epsilon(s)$.
%\textbf{Noise in reward: } In all experimental settings considered, noisy arms observe reward drawn from a perturbed reward function $\tilde{R}(s) = R(s)+\epsilon(s)$. %, where the noise $\epsilon(s)$ for each state $s$ is i.i.d. sampled from $\mathcal{N}(0,1)$. 

We evaluate our methods on the following domains. In all domains, 80\% of the arms are noisy, and noisy arms observe reward drawn from a perturbed reward function $\tilde{R}(s) = R(s)+\epsilon(s)$, where $\epsilon\sim\mathcal{N}(0,1)$. In ablation studies (Tables~\ref{table:num_noisy_arms_ablation} and~\ref{table:noise_shape_ablation}), we test various numbers of noisy arms and noise type. 

\textbf{Synthetic}: We consider a synthetic RMAB with continuous states. For state $s_{i}\in[0, 1]$ and action $a\in\{0,1\}$ of arm $i$, the next state $s_i'$ is determined by: $s_{i}' =  clip\left(s_i + \mathcal{N}(\mu_{ia}, \sigma_{ia}), 0, 1\right)$. Here transition parameters are sampled uniformly, specifically $\mu_{i1} = -\mu_{i0} \in [-0.2, 0.2]$, $\sigma_{i1} = \sigma_{i0} \in [0.1, 0.2]$.
% \[
% s_{i}' = \begin{cases} 
% \text{clip}\left(s_i + \mathcal{N}(\mu_{i0}, \sigma_{i0}), 0, 1\right) & \text{if } a = 0 \\
% \text{clip}\left(s_i + \mathcal{N}(\mu_{i1}, \sigma_{i1}), 0, 1\right) & \text{if } a = 1 \\
% \end{cases}
% \]
% \[
% \mu_{i0} \in [-0.2, -0.4], \quad \mu_{i1} \in [0.2, 0.4].
% \] 

\textbf{SIS\ Epidemic\ Model}~\cite{yaesoubi2011generalized,killian2022restless, zhao2024towards}: Each arm $p$ represents a subpopulation in a geographic region, with the number of uninfected individuals being the state $s_p$. We implement a budget-constrained intervention framework with three actions: \(a_0\) represents no intervention, \(a_1\) requires weekly COVID testing, and \(a_2\) involves distributing face masks. Actions change the disease transmission parameters in a targeted manner, reflecting their real-world public-health impacts. The reward noise is due to variability in data collection, which may be caused by poor COVID testing equipment \cite{embrett2022barriers,schmitt2020covid} and influence of authorities or impacted populations (keeping the COVID numbers low) \cite{paulus2023reinforcing}. 
% The transmission dynamics within each subpopulation are dictated by the average number of contacts $\kappa$, and the infection probability $r_{\textit{infect}}$ after contact.
% out of the total population $N_p$

\textbf{ARMMAN}: The dataset is collected by ARMMAN~\citep{armman-mhealth}, an NGO in India aimed at improving health awareness for a million expectant and new mothers via automated  voice messaging programs. Each arm represents a cluster of mothers in a geographical location. Actions are sending a health worker to visit mothers in a location to improve engagement. States, continuous valued in [0,1], represent the average engagement of mothers in a location ~\citep{danassis2023limited}. The transition dynamics is established empirically from the data (data usage and consent are in Appendix~\ref{sec:appendix_consent_data_usage}). Systematic reward errors are present due to difference in infrastructure such as cellular network and electricity \cite{kumar2022survey} (e.g. a geographic location may have poor cellular signals or frequent power outage, causing a systematic underestimation of mothers' engagement).  
%which affect a mother's ability to receive health message or to charge the phone, 






\textbf{Learning Performance}.\ \ Figure~\ref{fig:main_result_figure} shows the experimental results in \sname{Synthetic}, \sname{SIS}, and \sname{ARMMAN} where we compare our method \sname{Comm\ (Ours)} against various baselines and ablations. \sname{No\ Comm} is an ablation where the RMAB with noisy arms is trained without communication. \sname{Fixed\ Comm} involves a preset, fixed communication pattern where at each timestep, each noisy arm receives information from a similar ($\ell_2$ distance of features), noise-free arm. \sname{Fixed\ Comm} uses oracle information about which arms are noisy, which is not known by other methods. \sname{Nearest\ Neighbor\ Comm} is a baseline strategy where an arm always receives communication from the nearest neighbor in feature space, regardless of whether the sender/receiver is a noisy arm. We include \textbf{two additional baselines} in Tables~\ref{table:noise_level_ablation} and \ref{table:num_noisy_arms_ablation}. 
%\sname{Random} is a baseline strategy where the central planner selects actions randomly until the budget is depleted. 



% \begin{table*}[h!]
% \centering
% \scalebox{.99}{
%     \begin{tabular}{l@{}p{0.1mm}c ccc@{} c ccc@{} c ccc@{}}
%     \toprule
%     \multirow{1}{*}{} & \multirow{3}{*}{\ \ } & \multicolumn{3}{c}{\textbf{Synthetic (N=21, B=15)}} 
%      & & \multicolumn{3}{c}{\textbf{SIS (N=32, B=16)}}
%      & & \multicolumn{3}{c}{\textbf{ARMMAN (N=48, B=20)}}\\
%     \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
% \textbf{Method}& & \text{Gaussian} & \text{Uniform}  & \text{Mixture} & & \text{Gaussian}  & \text{Uniform} & \text{Mixture} & & \text{Gaussian}  & \text{Uniform} & \text{Mixture}\\
%     \midrule
%     \sname{No\ Noise} & & 100\%  & 100\%  & 100\% & & 100\%  & 100\%  & 100\% & & 100\% & 100\% & 100\%\\ 
%     \sname{Comm} & & 75\%  & 97\%  & 79\% & & 63\%  & 73\%  & 56\% & & 77\% & 100\% & 80\%\\  
%     \sname{No\ Comm} & & 62\%  & 92\%  & 71\% & & 55\%  & 66\%  & 47\% & & 63\% & 93\% & 75\%\\  
%     \sname{Fixed/ Comm} & & 21\%  & 15\%  & 16\% & & 56\%  & 29\%  & 27\% & & 24\% & 37\% & 35\%\\  
%     \sname{NN\ Comm} & & 44\%  & 89\%  & 62\% & & 32\%  & 48\%  & 20\% & & 46\% & 89\% & 72\%\\   
%     \sname{Random\ Comm} & & -24\%  & 21\%  & 1\% & & 22\%  & 24\%  & -1\% & & -22\% & 35\% & 28\%\\   
%   \bottomrule
%     \end{tabular}
% }
% \caption{Performance (return averaged across 100 random seeds) with various noise distributions, normalized with respect to \sname{No\ Noise} and \sname{Comm} (ours) before communication starts. Gaussian noise is $\mathcal{N}(0,1)$, Uniform noise is $U(-0.5,0.5)$, and Mixture noise has 50\% chance of being the Gaussian and 50\% chance of being the Uniform. We abbreviate 
% \sname{Nearest\ Neighbor\ Comm} as \sname{NN\ Comm} .}
% \label{table:noise_shape_ablation}
% \end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%


Our method significantly outperforms \sname{No\ Comm}, \sname{Fixed\ Comm}, and \sname{Nearest\ neighbor\ Comm}. Notably, the \sname{Fixed\ Comm} strategy, despite the oracle information, often performs worse than \sname{No\ Comm}. This observation aligns with our theoretical analysis in Proposition~\ref{prop:utor} showing that communication channels from non-noisy to noisy arms are not always helpful. 
%As the number of epochs increases, the communication pattern learnt by our method gradually improves and leads to a larger performance gap between our method and baselines. 
Our method consistently outperforms across various number of arms, budgets, and domains. For instance, in the Synthetic environment with N=21 and B=15, our method achieves a return of approximately 10 at epoch 600, compared to about 8 for the no communication (No Comm) baseline, representing an 20 percentage point improvement. Similarly, in the ARMMAN environment with N=48 and B=20, our method reaches a return of 15, outperforming the No Comm baseline's return of approximately 12.5, which is a 20 percentage point increase. 
These results demonstrate the effectiveness of our communication algorithm in handling systematic errors and enhancing learning in noisy RMAB environments.

\begin{figure}[h!]
\centering
    \includegraphics[width=0.45\textwidth]{figs/comm_pattern_figure.pdf}
    \caption{The change in the proportion of noise-free senders and receiver within all activated channels during the learning process. Results are for Synthetic (N=21, B=15), SIS (N=32, B=16), and ARMMAN (N=48,  B=16).}
    \label{fig:comm_pattern_figure}
\end{figure}


\begin{table*}[htb]
\centering
\scalebox{.9}{
    \begin{tabular}{l@{}p{0.1mm}c ccc@{} c ccc@{} c ccc@{}}
    \toprule
    \multirow{1}{*}{} & \multirow{3}{*}{\ \ } & \multicolumn{3}{c}{\textbf{Synthetic (N=21, b=15)}} 
     & & \multicolumn{3}{c}{\textbf{SIS (N=32, B=16)}}
     & & \multicolumn{3}{c}{\textbf{ARMMAN (N=48, B=20)}}\\
    \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
\textbf{Method}& & 100\% & 110\%  & 120\% & & 100\%  & 110\% & 120\% & & 100\%  & 110\% & 120\%\\
    \midrule
    \sname{No\ Noise} & & 100\%  & 100\%  & 100\% & & 100\%  & 100\%  & 100\% & & 100\% & 100\% & 100\%\\ 
    \sname{Comm} & & 75\%  & 53\%  & 38\% & & 63\%  & 55\%  & 51\% & & 77\% & 72\% & 68\%\\  
    \sname{No\ Comm} & & 62\%  & 39\%  & 24\% & & 55\%  & 45\%  & 42\% & & 63\% & 59\% & 52\%\\  
    \sname{Fixed/ Comm} & & 21\%  & 6\%  & 12\% & & 56\%  & 42\%  & 46\% & & 24\% & 15\% & 27\%\\  
    \sname{Nearest\ Neighbor\ Comm} & & 44\%  & 20\%  & 3\% & & 32\%  & 22\%  & 23\% & & 46\% & 43\% & 31\%\\   
    \sname{Random\ Comm} & & -24\%  & -45\%  & -58\% & & 22\%  & 13\%  & 9\% & & -22\% & -26\% & -35\%\\     
    \bottomrule
    \end{tabular}
}
\caption{Performance (return averaged across 100 random seeds) with increased noise levels, normalized with respect to \sname{No\ Noise} and \sname{Comm} (ours) before communication starts. We test Gaussian Noise $\mathcal{N}(0,\sigma)$, and the $x\%$ noise level means $\sigma=x/100$.}
\label{table:noise_level_ablation}
\end{table*}

\begin{table*}[htb]
\centering
\scalebox{.9}{
    \begin{tabular}{l@{}p{0.1mm}c ccc@{} c ccc@{} c ccc@{}}
    \toprule
    \multirow{1}{*}{} & \multirow{3}{*}{\ \ } & \multicolumn{3}{c}{\textbf{Synthetic (N=21, B=15)}} 
     & & \multicolumn{3}{c}{\textbf{SIS (N=32, B=16)}}
     & & \multicolumn{3}{c}{\textbf{ARMMAN (N=48, B=20)}}\\
    \cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
\textbf{Method}& & 15 & 16  & 17 & & 22  & 24 & 26 & & 34  & 36 & 38\\
    \midrule
    \sname{No\ Noise} & & 100\%  & 100\%  & 100\% & & 100\%  & 100\%  & 100\% & & 100\% & 100\% & 100\%\\ 
    \sname{Comm} & & 78\%  & 78\%  & 75\% & & 69\%  & 71\%  & 63\% & & 82\% & 80\% & 77\%\\  
    \sname{No\ Comm} & & 67\%  & 66\%  & 62\% & & 61\%  & 61\%  & 55\% & & 68\% & 59\% & 63\%\\  
    \sname{Fixed/ Comm} & & 63\%  & 45\%  & 21\% & & 65\%  & 62\%  & 56\% & & 43\% & 49\% & 24\%\\  
    \sname{Nearest\ Neighbor\ Comm} & & 42\%  & 47\%  & 44\% & & 11\%  & 29\%  & 32\% & & 47\% & 37\% & 46\%\\   
    \sname{Random\ Comm} & & -46\%  & -32\%  & -24\% & & -8\%  & 17\%  & 22\% & & -60\% & -30\% & -22\%\\   
   \bottomrule
    \end{tabular}
}
\caption{Performance (return averaged across 100 random seeds) with numbers of noisy arms, normalized with respect to \sname{No\ Noise} and \sname{Comm} (ours) before communication starts.}
\label{table:num_noisy_arms_ablation}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%



\textbf{Communication Pattern.} \ \ 
Figure~\ref{fig:comm_pattern_figure} illustrates how our learnt communication strategy evolves. We make several observations. First, as the number of learning epochs increase, we observe more information are sent from non-noisy arms to noisy arms. During the early stages of learning, when arms are primarily exploring, communication from noisy arms to non-noisy arms can be beneficial, as shown in Proposition~\ref{prop:utor}. As the learning progresses, the information from noisy sources may become less helpful as the arms have explored sufficiently. As a result, the proportion of communication from non-noisy arms increases. This observation is consistent across the three experimental environments. 

Second, notice the percentage of noise-free receivers do not drop to zero and noise-free senders are not at 100\% even at the end of training, indicating value of communication from noisy arms. Finally, the differing rates of noise-free arms as senders and receivers across domains indicate that our communication approach adapts to the domain. 


\textbf{Robustness.}\ \ Tables~\ref{table:noise_level_ablation} and ~\ref{table:num_noisy_arms_ablation} show the performance of different methods under various settings (see Appendix for more ablations). In \sname{No\ Noise}, all arms receive accurate, true reward signals without any noise. Arms learn individually on their own data without any communication. In \sname{Random\ Comm}, each arm receives communication from a randomly chosen arm. The results demonstrate that our method is robust under increasing noise levels, numbers of noisy arms, and different noise distributions. In contrast, the performance of baselines \sname{No\ Comm} and \sname{Fixed\ Comm} changes significantly when the environment changes. In particular, on Synthetic, when the number of noisy arms increases from 15 to 17 (Table~\ref{table:num_noisy_arms_ablation}), our \sname{Comm} method has \textbf{only 3\%} drop in performance, 
while \sname{Fixed\ Comm} has 42 percentage points drop in performance, despite that \sname{Fixed\ Comm} uses ground truth information about which arms are noisy that is not known to our \sname{Comm} method. Similar trends can be seen on SIS and ARMMAN. These results demonstrate that, compared to a fixed communication protocol with access to oracle information, our approach for communication learning 
%enhances the ability to deal with a larger variety of tasks and thus 
provides better robustness. Additionally, the performance of \sname{No\ Comm} supports the argument that conventional RL methods struggle in noisy RMABs.






==> text/5-Conclusion.tex <==
\section{Closing Remarks}

The study of RMABs in environments with noisy and unreliable data sources underscores the need for innovative solutions in RL methods. 
%In this paper,
We introduce a novel communication learning algorithm to alleviate the influence of noisy data so that the central planner can make better coordination decisions. 
%We theoretically derive the condition under which communication can help reduce errors in value function approximation and 
Theoretically, we prove that communication can help reduce errors in value function approximation if the behavioral policy's state-action occupancy probability is lower bounded by a suitable constant. Empirically, we show that our approach significantly improves RMAB 
performance. Our findings advance the understanding of RMAB dynamics and enhance their applicability across real-world settings. 
%, setting a new standard for future algorithm development in the field.

% We envision this work to have notable real-world implications, particularly in enhancing decision-making processes in environments with noisy data, such as public health interventions. By introducing a novel communication learning algorithm, the study enables more effective resource allocation and policy development, leading to improved outcomes in healthcare and epidemic prevention by allowing agents to correct and optimize their actions based on collective information. We hope this work can contribute to more resilient and adaptable systems in practical applications where data reliability is often compromised.

==> text/backup.tex <==
% %%%% Method, Version 05/10/16:00
% %%%% This version has two lemmas to explain the difficulty of the communication. Plan to change this to example + proposition.

\section{RMAB Learning with Communication}

In this section, we introduce our method of learning communication to share useful knowledge among arms. Our framework addresses the following critical design and learning problems: (1) Message design: what are the messages sent between arms that are informative? (2) Communication reward design: how to generate reward signals that can measure the influence of communication? (3) Learning design: how to use the communication reward to learn a good communication protocol? 

% (4) Robustness design: how to deal with the influence of random rewards in each arm on communication learning? In Sec.~\ref{sec:alg_com}, we answer these four questions and describe the details of communication learning. In Sec.~\ref{sec:alg_all}, we describe the overall RMAB learning with communication algorithm, addressing the problem of how to interleave communication learning and policy learning for each arm.

\subsection{The Communication Learning Problem}

Akin to traditional deep RMAB learning algorithms, our approach involves each arm learning its local Q networks $Q_i(s_i, a_i; \theta_i)$ to predict the expected return of taking action $a_i$ in state $s_i$. The central planner then makes centralized action selections based on the combined Q values. However, when the data source is unreliable, e.g., if the reward signals from some arms are noisy, the local Q functions may be inaccurate, leading to the central planner choosing suboptimal actions.

To address this issue, we introduce a mechanism that allows the arms to learn a communication policy that diminishes the impact of unreliable data and enhances the overall effectiveness of the central planner. To describe our method, we first define the communication learning problem within the framework of a Multi-Agent MDP~\cite{boutilier1996planning}.
\begin{definition}[The Communication MDP]
    The communication MDP in the RMAB setting is a multi-agent game modelled by a multi-agent MDP $\mathcal{M}^\texttt{c}=(\mathcal{S}^\texttt{c}, I, \mathcal{A}^\texttt{c}, T^\texttt{c}, \comr)$. $I$ is the set of players, which in our case is the set of communication channels. Each state $\coms \in \mathcal{S}^\texttt{c}$ is a parameter profile of the arms' Q-functions $\bm\theta=(\theta_1,\cdots,\theta_N)$. Each player chooses an action from the binary action set $\mathcal{A}^\texttt{c}$, where 1 means the communication channel is activated. The joint communication action $\jcoma$ leads to a transition in $\bm\theta$ and a reward $\comr$.
\end{definition}
\dn{ An MDP requires the following things to be completely defined completely. Currently, these things are spread out over the sections. If we can either define them at one place or reference where they are defined, it would be helpful:
\begin{enumerate}
    \item State space
    \item Action Space
    \item Reward for a given state and action
    \item state evolution given action.
\end{enumerate}
Some more comments:
In the Definition above, explicitly define $\mathcal{S}^{\texttt{c}} = \Theta^{I}$ where $\Theta$ is the parameter space of a single Q network. That is, $\bm\theta = (\theta_1,\dots,\theta_N) \in \mathcal{S}^{\texttt{c}}$ where $\theta_i$ corresponds to the current Q-function parameter of arm $i$.
  $\mathcal{A}^{\texttt{c}} = \{0,1\}^{I}$. The action $(a^{\texttt{c}}_1,\dots,a_N^{\texttt{c}}) \in \mathcal{A}^{\texttt{c}}$ is such that $a^{\texttt{c}}_{i} = 1$ means arm $i$ decides to obtain Q-value parameters from its nearest arm $\nu_i$.   }
The definition of this Communication MDP is associated with the underlying RMAB problem.  We assume that each arm $i$ in the system has the chance to communicate with other arms. For arm $i$, there is a communication channel linked from the arm with the most similar feature, denoted by arm $\senderfor{i}$. Each arm needs to choose an communication action $\coma{i}$. If $\coma{i}$ is 1, the communication channel is activated, otherwise it remains inactive.

Therefore, there are $N$ communication channels in our system, which comprise the set of players in the Communication MDP. In the following proposition, we show that there is no need to consider a denser communication network, such as one with a channel between every pair of arms.
\begin{proposition}[Sparse Communication]
\tw{@Dheeraj: If you want to add a theorem about the sparity of communication channels, please insert it here.}    \dn{Will write down the result here, we can move it to an appropriate place later. This needs to appear after we have defined the gradient descent step.}

\end{proposition}
\dn{
We now show that given a dense communication strategy, we can have a sparse communication strategy which approximates the optimization step in Equation~\eqref{equ:coms_t} faithfully. 

Suppose we consider dense communication, where the arm $i$ communicates with $d$ similar arms $\senderfor{i,1},\dots,\senderfor{i,d}$. In this case, the arm collects data from each of the policies $\mathcal{D}_{\pi_{\senderfor{i,1}}},\dots, \mathcal{D}_{\pi_{\senderfor{i,d}}}$. We call this mixture distribution $\bar{\mathcal{D}}_{i}$. Now, consider the TD-loss for this dense communication: 
\begin{align}
\mathcal{L}^\texttt{c,dense}_\texttt{TD}(\theta_i|\coma{i}\shorte 1) = \mathbb{E}_{(s_i, a_i, s_i')\sim\bar{\mathcal{D}}_{i}}\left[\left(R(s_i)-\lambda c_{a_i} + \beta \max_a Q_i(s_i',a;\theta_i)-Q_i(s_i,a_i;\tilde{\theta}_i)\right)^2\right].
\end{align}
Now, suppose that we pick a random variable $J$ uniformly at random from $\{1,\dots,d\}$ and collect data only from the arm $\nu_{i,J}$. Then, we define:
\begin{align}
\mathcal{L}^\texttt{c,sparse}_\texttt{TD}(\theta_i|\coma{i}\shorte 1) = \mathbb{E}_{(s_i, a_i, s_i')\sim\mathcal{D}_{\senderfor{i,J}}}\left[\left(R(s_i)-\lambda c_{a_i} + \beta \max_a Q_i(s_i',a;\theta_i)-Q_i(s_i,a_i;\tilde{\theta}_i)\right)^2\right].
\end{align}
Then, we have:
\begin{align}
    \mathcal{L}^\texttt{c,dense}_\texttt{TD}(\theta_i|\coma{i}\shorte 1) &= \mathbb{E}[ \mathcal{L}^\texttt{c,sparse}_\texttt{TD}(\theta_i|\coma{i}\shorte 1)] \nonumber \\
 \nabla\mathcal{L}^\texttt{c,dense}_\texttt{TD}(\theta_i|\coma{i}\shorte 1) &= \mathbb{E}[\nabla  \mathcal{L}^\texttt{c,sparse}_\texttt{TD}(\theta_i|\coma{i}\shorte 1)] \label{eq:stoc_approx}
\end{align}

Now consider the gradient descent (GD) in Equation~\eqref{equ:coms_t} with $\mathcal{L}^\texttt{c,dense}_\texttt{TD}(\theta_i|\coma{i}\shorte 1)$. When this loss is replaced with $\mathbb{E}[ \mathcal{L}^\texttt{c,sparse}_\texttt{TD}(\theta_i|\coma{i}\shorte 1)]$, it becomes stochastic gradient descent (SGD) for $\mathcal{L}^\texttt{c,dense}_\texttt{TD}(\theta_i|\coma{i}\shorte 1)$. SGD is widely deployed to optimize loss functions in deep learning since GD is much more expensive \cite{bottou2010large}. It can be shown that for a large class of loss functions, SGD converges to the same optimal solution as GD \cite{robbins1951stochastic,polyak1992acceleration}. Notice that even in our case, we reduce the computational complexity per-step by a factor of $O(d)$. 
}
\subsection{Communication Actions and Transition Dynamics}~\label{sec:alg_com}
We now explain how the communication action $\jcoma$ induces a transition in the state space $\mathcal{S}^\texttt{c}$.

When $\coma{i}$ is 1, arm $i$ receives a message from arm $\senderfor{i}$, which is the parameters of the local Q network of arm $\senderfor{i}$. \tw{Not sure whether we need to say more to support this design choice.} 
\dn{We should definitely say more about this design choice since it is not clear to a reader without reading the rest of the paper. A toy example would be sufficient I think: I was thinking of the tree example where some of the intermediate states have small misleading rewards whereas the goal state reward is large.}
On receiving the message, arm $i$ establishes a behavior policy $\pi_{{\senderfor{i}}}$ based on this Q function $Q_{\senderfor{i}}$:
\begin{align}
    \pi_{b_{\senderfor{i}}}(\cdot|s_i)=\texttt{SoftMax}\left(Q_{\senderfor{i}}(s_i,\cdot)\right).
\end{align}
Arm $i$ uses this behavior policy to walk in the arm MDP $\mathcal{M}_i$ and collect a replay buffer $\mathcal{D}_{\pi_{\senderfor{i}}}$ consisting of transition samples, which is further used to update the local Q-network. Therefore, the TD-loss for arm $i$ with the communication channel $i$ activated is:
\begin{align}
\mathcal{L}^\texttt{c}_\texttt{TD}(\theta_i|\coma{i}\shorte 1) = \mathbb{E}_{(s_i, a_i, s_i')\sim\mathcal{D}_{\pi_{\senderfor{i}}}}\left[\left(R(s_i)-\lambda c_{a_i} + \beta \max_a Q_i(s_i',a;\theta_i)-Q_i(s_i,a_i;\tilde{\theta}_i)\right)^2\right].
\end{align}
% If multiple messages are received by arm $j$, we use their average:
% \begin{align}
% \mathcal{L}^\texttt{c}_\texttt{TD}(\theta_j|\jcoma) = \mathbb{E}_{(s_j, a_j, s_j')\sim\mathcal{D}}\left[\left(R(s_j)-\lambda c_{a_j} + \beta \max_a \sum_{i:\coma{i}{j}=1}Q(s_j',a;\theta_i)-Q_j(s_j,a_j;\theta_j)\right)^2\right].
% \end{align}
% where $\jcoma$ is the joint communication action consisting of all $\coma{i}{j}$. 
In the case arm $i$ chooses to not communicate, it uses $\epsilon$-greedy strategy to explore the MDP $\mathcal{M}_i$ to generate the replay buffer. 

Therefore, the changes in local Q parameters are dependent on the communication action:
\begin{align}
    \theta_i'(\coma{i}) = \theta_i - \alpha\nabla_{\theta_i}\mathcal{L}^\texttt{c}_\texttt{TD}(\theta_i|\jcoma),\label{equ:coms_t}
\end{align}
where $\alpha$ is the learning rate. Eq.~\ref{equ:coms_t} specifies the state transition dynamics in the Communication MDP.

\subsection{Learn Communication}
Intuitively, an active communication channel from a reliable arm to an unreliable arm might seem beneficial, as it allows for the collection of learning samples using a behavior policy free from reward noise. Conversely, it might seem logical to deactivate the communication channel from an unreliable arm to a reliable arm. However, the following lemmas demonstrate that the reality may be counter-intuitive.

We first show that if the MDP associated with a reliable arm is too different from the MDP in an unreliable arm, the communication might lead to larger errors in the local value function.
\begin{lemma}[Reliable to Unreliable Communication can be Harmful]\label{prop:rtou}
    Suppose that the data source of arm $i$ is unreliable and that its rewards suffer from noise: $\max_{s_i}|\epsilon_i(s_i)|\le\epsilon$. When the noise is smaller than a threshold
    \begin{align}
        \epsilon<\epsilon_R+\frac{\gamma}{1-\gamma}\epsilon_PR_{max},
    \end{align}
    using optimal policy from arm $\senderfor{i}$ as a behavior policy leads to a larger error in the value function than that induced by noise in arm $i$. Here, $\epsilon_R$ and $\epsilon_P$ are the upper bounds of the difference in the reward function and transition probability, respectively: $\max_{s}|R_i(s)-R_{\senderfor{i}}(s)|\le\epsilon_R$, $\max_{s,a,s'}\|T_i(s,a,s')-T_{\senderfor{i}}(s,a,s')\|_1\le\epsilon_P$.
\end{lemma}
We then show that even if an arm has a noisy reward function, using its noisy Q function to establish a behavior policy can help the exploration of another reliable arm. To discuss the conditions where this is applicable, we define the minimum state-action occupancy probability
\begin{align}
    \mu_{\texttt{min}} := \min_{s,a}\mu_{\pi_{\nu_i}}(s,a),
\end{align}
and the mixing time~\cite{hsu2015mixing,li2020sample}
\begin{align}
    t_\texttt{mix} = \min\left\{t|\max_{s_0,a_0}\sup_{s,a} |P^t(s,a|s_0,a_0)-\mu_{\pi_{\nu_i}}(s,a)|\le\frac{1}{4}\right\},
\end{align}
where $P^t$ is the state-action distribution at timestep $t$ given the initial state and action. $t_\texttt{mix}$ captures how fast the behavior policy decorrelates from the initial state.

\begin{lemma}[Unreliable to Reliable Communication can be Useful]\label{prop:utor}
When
\begin{align}
    \mu_{\texttt{min}}>\frac{2(1-\gamma)^2}{|\mathcal{S}||\mathcal{A}|},\ \ \text{and}\ \ t_\texttt{mix}\le \frac{1}{\epsilon^2(1-\gamma)^4},
\end{align}
for any $0<\delta<1$, with a probability at least $(1-\delta)^2$, compared to learning without communication, using behavior policy $\mu_{\pi_{\nu_i}}$ leads to better sample complexity in the worst case in learning $\epsilon$-optimal Q function such that $\|Q_i(s,a)-Q_i^*(s,a)\|<\epsilon, \forall (s,a)$.
\end{lemma}

% Proposition~\ref{prop:rtou} indicates that incorporating messages from a reliable arm into an unreliable arm can be detrimental, particularly when the inherent noise of the unreliable arm is less than the impact of differences between their respective MDPs. Conversely, Proposition~\ref{prop:utor} establishes that messages from an unreliable arm can be beneficial to a reliable arm, as they may enhance exploration when the behavior policy is ergodic.

Lemma~\ref{prop:utor} establishes that when the behavior policy visits every state-action pair with a positive probability and is not too slowly in disentangling from the initial state, communication can accelerate Q-learning, possibly by providing a better exploration strategy.

Together, these two lemmas highlight the complexity of the communication learning problem within the RMAB framework. Under certain conditions, a seemingly intuitive and fixed communication pattern does not effectively address the issue of data unreliability.

% To decide whether arm $i$ should communicate with arm $j$, we need to estimate the utility of the activation of this communication channel, which is measured by a channel-level communication Q-function $\comQ{i}{j}$. 
To tackle this problem, we propose that each arm learns a communication Q function $\comQ{i}$ to dynamically decide the best communication action. The challenge is that, in the RMAB setting, there is no clear, separate reward signal for each $\comQ{i}$ because the planner policy chooses action based on the updated Q-functions of all arms and the budget. Consequently, what we can measure is the collaborative contribution of the joint communication action $\jcoma$ to the learning objective:
\begin{align}\label{equ:comm_r}
    \comr(\bm\theta,\jcoma) = G_T\left(\pi(\bm\theta'(\jcoma))\right) - G_T\left(\pi(\bm\theta'(\bm 0))\right).
\end{align}
Here, $G_T(\pi)$ is the empirical return under policy $\pi$ averaged over $T$ episodes:
\begin{align}
    G_T(\pi) = \frac{1}{T}\sum_{k=1}^T\left[\sum_{t=1}^H \beta^t\sum_{i\in[N]}R_i(s_i^{k,t})\right],
\end{align}
where $s_i^{k,t}$ is the state of arm $i$ at timestep $t$ of the $k^{\text{th}}$ episode. $\pi(\bm\theta'(\jcoma))$ and $\pi(\bm\theta'(\bm 0))$ are the planner policies with the arm Q-functions updated with and without messages, respectively, and the communication reward is defined as the difference in the planner's return in this two cases.

% The question is how to train this communication Q-function. Intuitively, we need a reward signal that captures the contribution of the communication action $\coma{i}{j}$ to the learning objective. However, . The reason is that, our learning objective is to maximize the accumulated return from the opted-in arms. All communication actions will \emph{together} influence the opt-in decisions, and then influence the global learning objective. 

% As a result, what we have is a \emph{global} communication reward


\subsection{Decomposed Communication Q Function}
The definition of the communication reward (Eq.~\ref{equ:comm_r}) enables the usage of Q-learning to learn the communication policy. The simplest strategy is to estimate a deep communication action-value function $\jcomQ(\bm\theta, \jcoma)$ for the communication MDP. However, the question is that there are $N$ communication channels, and even though our communication action is binary, there are $2^{N}$ possible $\jcoma$. With this exponential number of actions, it is challenging to use Q-learning to train $\jcomQ$, which requires a maximization operation over the whole action space.


% $\coms$ is the state of the communication Q-function. By observing that the communication reward is defined on the parameters of arms' Q-functions and that the communication action leads to a transition between two parameter vectors of the arms' Q-functions, the state of the communication Q-function should be the joint parameter of the arms' Q-functions, $\bm\theta$. That is, we have
% \begin{align}
%     \coms\in \mathcal{S}^\texttt{c} = \Theta 
% \end{align}

We propose to solve this problem by value decomposition. Specifically, we learn the global communication Q-function as a summation of the channel-level communication Q-functions:
\begin{align}
    \jcomQ(\bm\theta, \jcoma;\bm\xi) = \sum_{i\in[N]}\comQ{i}(\bm\theta, \coma{i};\xi_{i}).
\end{align}
Here, $\xi_{i}$ is the parameters of the channel-level communication Q-function, and $\bm\xi$ is the joint parameter consisting of all $\xi_{ij}$. This linear decomposition of $\jcomQ$ effectively learns (how to establish) a credit assignment scheme that decomposes the joint reward into utilities of all communication actions. 

The decomposed Q-network is updated by the gradients of the TD-loss
\begin{align}
\mathcal{L}^\texttt{d}_\texttt{TD}(\bm\xi) = \mathbb{E}_{(\bm\theta,\jcoma,\bm\theta')\sim\mathcal{D}}\left[\left(\comr(\bm\theta,\jcoma) + \gamma \max_a \jcomQ(\bm\theta', a; \tilde{\bm\xi})-\jcomQ(\bm\theta,\jcoma;\bm\xi)\right)^2\right].
\end{align}
$\jcomQ(\cdot; \tilde{\bm\xi})$ is a target network with parameters periodically copied from $\jcomQ$, and $\mathcal{D}$ is a replay buffer.

% \textbf{Dealing with noise}.\ \ [Change the communication Q function to distributional. Prove that it still conforms to IGM. Write this after obtaining experimental results.]

% 
% % \subsection{Overall Learning Framework}~\label{sec:alg_all}


% V of different policies in the same MDP

\subsection{Lemma~\ref{prop:rtou}}

We analyse two arms $i$ and $j$. The MDPs associated with these two arms are $M_i=(\mathcal{S}, \mathcal{A}, \mathcal{C}, T_i, R_i,\beta, \bm z_i)$ and $M_j=(\mathcal{S}, \mathcal{A}, \mathcal{C}, T_j, R_j,\beta, \bm z_j)$. We denote the upper bound of the difference in the reward function by
\begin{align}
    \max_{s}|R_i(s)-R_j(s)|\le\epsilon_R,
\end{align}
and the upper bound of the difference in the transition probability by
\begin{align}
    \max_{s,a}\|P_i(s,a)-P_j(s,a)\|_1\le\epsilon_P.
\end{align}

\begin{lemma}
    For any policy $\pi$ and two MDPs associated with arm $i$ and $j$, we have
    \begin{align}
        \|V_{M_i}^\pi-V_{M_j}^\pi\|_\infty\le \frac{\epsilon_R}{1-\gamma}+\frac{\gamma\epsilon_PR_{max}}{(1-\gamma)^2}.
    \end{align}
\end{lemma}
This lemma enables us to analyse what will happen when we use the optimal policy of $M_i$ to another arm $M_j$.
\begin{lemma}
    When applying the optimal policy on MDP $M_j$, $\pi^*_{M_j}$, to $M_i$, it follows that
    \begin{align}
        V_{M_i}^*(s) - V_{M_i}^{\pi^*_{M_j}} \le 2\left[\frac{\epsilon_R}{1-\gamma}+\frac{\gamma\epsilon_PR_{max}}{(1-\gamma)^2}\right]
    \end{align}
\end{lemma}
Now we can get the condition under which communication can help a noisy arm learn better:
\begin{lemma}
    Suppose that rewards of arm $i$ suffer from noise and $\max_{s}|R_i(s)-R_i'(s)|\le\epsilon$, when the noise is larger than a threshold
    \begin{align}
        \epsilon>\epsilon_R+\frac{\gamma}{1-\gamma}\epsilon_PR_{max},
    \end{align}
    use optimal policy from arm $j$ as a behavior policy can reduce the influence of noise on the optimal value function.
\end{lemma}


% %%%%% Introduction version May 17 3pm China Time

\section{Introduction}

Restless Multi-Arm Bandits (RMABs) is a multi-agent reinforcement learning (RL) problem where the agents' actions are constrained by global resource constraints. This model has been successfully applied across a range of real-world problems, such as resource allocation in multi-channel communication, machine maintenance, and healthcare~\cite{ruiz2020multi,bhattacharya2018restless,lee2019optimal,hodge2015asymptotic,mate2022field,modi2019transfer,zhao2007myopic,bagheri2015restless,tripathi2019whittle}.  While the exact solution to RMAB is known to be PSPACE-hard~\cite{papadimitriou1994complexity}, there are many successful approximation algorithms which achieve strong performance. In a classical RMAB, there are a fixed number of arms, each associated with a fixed and known Markov Decision Process (MDP) with two actions (active and passive) with a global constraint on the number of active actions played in each step. At each timestep, the RMAB selects a subset of arms to play the active action so that the long-term accumulated reward from all the arms is maximized. In this situation, the whittle index solution is known to be near optimal~\cite{whittle1988restless,weber1990index}.

Important applications of RMABs involve more complex systems with multiple-actions, continuous state spaces and agents/arms opting in and out of the system. Recent works have explored extensions of whittle index \cite{hawkins2003langrangian,killian2021beyond}, convex relaxations \cite{verloop2016asymptotically,zayas2019asymptotically,ghosh2023indexability} and Deep RL in order to tackle these scenarios \cite{zhao2023towards,xiong2023finite,wang2023scalable,killian2022restless}. These works consider systems where the state, action and reward data can be collected from every arm (or agent) reliably. In real world scenarios, such data could be collected from multiple sources where some arms have systematic error in their reward data. We can consider the example of healthcare where multiple organizations, each involving multiple beneficiaries must be allocated funds from a global source. Some of these organizations can potentially have non-standard collection procedures or the beneficiaries can possibly misrepresent their information. Some organizations can have strict differential privacy rules which disallow sharing of exact data.


% Current experimental set up: At optimal states, we always observe the true reward, and once we arrive at optimal states we will stay there for a prolonged period of time. That is how we get the correct signal to update communication strategies.

We give specific motivations based on the datasets we consider for empirical examples. (1) The ARMMAN dataset deals with maternal healthcare, where resources have to be allocated to ensure expectant mothers have access to relevant healthcare information. Here, each arm may represent a geographical location. There might be significant geographical differences in infrastructure such as availability of internet connections or access to mobile phones. Thus, data collected from some arms could be noisy/unreliable. (2) The epidemic modeling example considers the spread of diseases in a population. In this situation, each arm may represent a city. The quality of data from each city might be different due to differences in testing equipments and data collection policies. For example, certain testing and quarantining policies for Covid could motivate people to misrepresent their symptoms. (3) When data is collected by surveys, these might come with strict data privacy laws. Some respondents might opt out of sharing detailed information. In such instances noise can be intentionally added to the reward data in order to achieve differential privacy \cite{dwork2014algorithmic}. 



Motivated by these scenarios, we consider the problem of learning RMAB policies where some arms have a \textbf{systematic error} in their reward signals (which we call noisy arms). We do not assume that the identity of the noisy arms are known apriori. In contrast, Multi-Armed Bandits and RL literature \cite{sutton2018reinforcement,lattimore2020bandit} consider \textbf{random errors} where rewards are observed with a zero-mean, independent, additive error at every observation. In the case of random errors, averaging over multiple observations can lead us to the correct rewards and most RL and Bandit algorithms are designed to converge in this scenario. However, systematic errors we consider need not be zero mean or independent. 


An example of this scenario is that of Reinforcement Learning with Human Feedback (RLHF). Here human preference data is used to directly build a reward model and use the reward model to train LLMs which align with these preferences \cite{ouyang2022training,askell2021general}. Revealing the rewards exactly might leak confidential information collected from human subjects and thus differentially private methods for RLHF have been explored (\cite{chowdhury2023differentially,wu2023privately}). One proposal in this case (\cite{wu2023privately}) is to reveal a noisy version of the reward model. Such a method can use the Laplace Mechanism (\cite{dwork2014algorithmic}) which reveals a data vector (such as reward corresponding to a state-action pair) by adding a noise vector from the Laplace distribution. This noise is sampled once, making it systematic since averaging over multiple DP queries does not allow us to reconstruct the exact reward vector. 

In the case of RMABs, noisy arms with systematic error might learn the wrong Q functions in case they are trained exclusively on their own data, leading to bad policies being learned. In order to mitigate this, we allow the arms to communicate aggregate information like Q function parameters with other arms. This allows a noisy arm to communicate in order to collect aggregate data from other arms similar to itself, augment its own collected data and learn the correct policy for itself. However, since the identity of the noisy arms are unknown aprori, we design a novel communication learning algorithm which automatically learns which arms should communicate with each other during the training of RMABs. 

\textbf{Our Contribution} is threefold. (1) We consider the setup of learning RMABs where some arms collect systematically unreliable reward data and show empirically that the currently popular RMAB algorithms are ineffective in this scenario. (2) We design a novel communication learning algorithm, where arms learn to share information with each other during the RMAB training. This allows noisy arms to identify and collect useful data from similar arms to learn the correct policy for itself. Here RMAB training with communication itself is re-cast as a multi-agent RL problem. The rewards are then computed as the joint utility of the messages and then decomposing it to understand the payoff of each communication between each pair of arms. (3) We validate the effectiveness of our method through both theoretical analysis and empirical results, demonstrating its capability to significantly improve RMAB performance across diverse problems.


\subsection{Related Works}

Recent works in RL and online learning have considered multiple agents collaboratively exploring in order to learn their respective optimal policies \cite{nagaraj2023multi,bresler2021regret,ariu2020regret,pal2024blocked,lei2019collaborative}. Here, the algorithms are designed to identify agents/arms which are most similar and share data in order achieve better performance than a single agent exploring the entire environment. \cite{zhao2023towards} considers RMABs where arms can opt-in and drop-out at test time. Therefore, a neural network based policy is trained to generalize to unseen arms at test time, given their features by using the data from known arms during training.  

In the literature of cooperative multi-agent reinforcement learning~\cite{yu2022surprising,wen2022multi,kuba2021trust,wang2020roma,christianos2020shared,peng2021facmac,wang2020dop,jiang2019graph}, value decomposition methods~\cite{sunehag2018value,rashid2018qmix,son2019qtran,li2021celebrating} have recently witnessed great success in addressing challenges such as partial observability and learning scalability. In these methods, each agent has a local Q function based on local action-observation history and local actions. The joint Q value conditioned on true states and joint actions is learned to be a combination of local Q values. In this work, we adopt a linear value decomposition framework~\cite{sunehag2018value} for the communication Q network to deal with the credit assignment problem there. 

% RMABs are a specific instance of the powerful multi-agent RL framework used to model systems with multiple interacting agents in both competitive and co-operative settings \cite{shapley1953stochastic,littman1994markov}, for which significant strides have been made empirically \cite{jaques2019social,yu2022surprising} and theoretically \cite{jin2021v,xie2020learning}. \cite{nakhleh2021neurwin} proposed a deep RL method to estimate the Whittle index. \cite{fu2019towards} provided an algorithm to learn a Q-function based on  Whittle indices, states, and actions. \cite{avrachenkov2022whittle} and \cite{biswas2021learn} developed Whittle index-based Q-learning methods with convergence guarantees. While the aforementioned works focus on binary action RMABs, \cite{killian2021q} generalized this to multi-action RMABs using tabular Q-learning. A subsequent work \cite{killian2022restless}, which focussed on robustness against adversarial distributions, took a deep RL approach that was more scalable. However, existing works on multi-action RMABs do not consider streaming RMABs and require training from scratch when a new arm opts-in. Additionally, works built on tabular Q-learning \cite{fu2019towards,avrachenkov2022whittle,biswas2021learn,killian2021q} may not generalize to continuous state RMABs without significant modifications. Our pretrained model addresses these limitations, and enables zero-shot ability on a wide range of unseen RMABs.

% The community has long been intrigued by the challenge of enhancing learning efficiency in RMABs beyond developing approximate algorithms~\cite{hawkins2003langrangian,whittle1988restless}. Notably, the potential to reuse useful knowledge from other arms offers a promising revenue to achieve this goal. The underlying intuition is that certain arms may acquire valuable knowledge more quickly. This allows them to share their local insights with other arms that have similar reward and transition dynamics but are learning at a slower pace.

% An example scenario where communication can be particularly useful is in RMABs with certain arms have noisy reward functions. This scenario represents an important class of resources allocation problem. For example, in [xxx task], the reward is noisy [xxx]. Establishing a communication channel from a noise-free arm to other noisy arms with similar a MDP structure holds the promise to help noisy arms eliminate the influence of noise. However, how to identify these beneficial communication channels is still an open question.

% In this paper, we tackle this long-standing problem and develop a communication learning algorithm among arms in RMABs. Considering the real-world applications of this type of algorithm, it is a priority to safeguard the privacy of each arm. To this end, the messages cannot be specific information. Instead, they can contain statistic information about the arm. We propose that Q-values is a good type of messages that can preserve privacy. This is because []. Therefore, in our method, 

% we propose using the Q-function of an arm as the potential message to be sent to other arms. This approach is feasible because Q-values function as a type of statistic. Under this communication protocol, our focus shifts to discovering effective communication channels.



% %%%%% May 20 3pm China time. Proposition 2 in the method section
% We first show that if the MDP associated with a reliable arm is too different from the MDP in an unreliable arm, the communication might lead to larger errors in the local value function.
% \begin{lemma}[Reliable to Unreliable Communication can be Harmful]\label{prop:rtou}
%     Suppose that the data source of arm $i$ is unreliable and that its rewards suffer from noise: $\max_{s_i}|\epsilon_i(s_i)|\le\epsilon$. When the noise is smaller than a threshold
%     \begin{align}
%         \epsilon<\epsilon_R+\frac{\gamma}{1-\gamma}\epsilon_PR_{max},
%     \end{align}
%     using optimal policy from arm $\senderfor{i}$ as a behavior policy leads to a larger error in the value function than that induced by noise in arm $i$. Here, $\epsilon_R$ and $\epsilon_P$ are the upper bounds of the difference in the reward function and transition probability, respectively: $\max_{s}|R_i(s)-R_{\senderfor{i}}(s)|\le\epsilon_R$, $\max_{s,a,s'}\|T_i(s,a,s')-T_{\senderfor{i}}(s,a,s')\|_1\le\epsilon_P$.
% \end{lemma}
% We then show that even if an arm has a noisy reward function, using its noisy Q function to establish a behavior policy can help the exploration of another reliable arm. To discuss the conditions where this is applicable, 


% Proposition~\ref{prop:rtou} indicates that incorporating messages from a reliable arm into an unreliable arm can be detrimental, particularly when the inherent noise of the unreliable arm is less than the impact of differences between their respective MDPs. Conversely, Proposition~\ref{prop:utor} establishes that messages from an unreliable arm can be beneficial to a reliable arm, as they may enhance exploration when the behavior policy is ergodic.
